Neutron Scattering studies of the density dependence of One-dimensional Quantum Fluids

In previous work, we demonstrated that $^4$He confined within a templated porous material preplated with a noble gas to enhance dimensional reduction exhibits one-dimensional behavior. Neutron scattering revealed that the excitations in confined $^4$He are qualitatively distinct from those in two- and three-dimensional superfluid helium, aligning with quantum Monte Carlo calculations. These simulations suggest that three solid layers form, with a one-dimensional liquid located at the center of the pore. Here, we present neutron scattering results as the filling fraction of the one-dimensional core is varied. We observe that the one-dimensional liquid always forms with a fixed density, even as the pore filling increases. We posit that this is due to the growth of the one dimensional extent of the liquid as the filling is increased, but its density remains unchanged.

==> snippets.tex <==
\section{Text snippets}

we can effectively reduce the pore diameter, allowing confined $^4$He to enter the Luttinger liquid regime. I

We have recently developed a nanoengineering technique that enables us to observe Luttinger liquid behavior in $^4$He. By preplating the pores of a templated glass with argon at high temperatures, we can effectively reduce the pore diameter, allowing confined $^4$He to enter the Luttinger liquid regime. In this paper, we will review previous studies of confined $^4$He that led to the observation of Luttinger liquid behavior in liquid helium.\\


There are numerous systems where the two- and three-dimensional dynamics have been explored.  In these systems, the behavior is well-described by quasiparticles with renormalized properties. The physics changes fundamentally in one spatial dimension (1D). In 1D, excitations are inherently collective and at long wavelengths and low energies, the system is governed by the linear hydrodynamics of Tomonaga-Luttinger liquid (TLL) theory [3–8]. In one dimension, the significance of exchange interactions profoundly affects particle statistics, bluring the distinction between bosonic and fermionic isotopes, making 1D helium an excting system to study.\\


\noindent
In contrast, helium should enable continuous adjustment of the Luttinger parameter across its entire range, allowing us to investigate the model’s behavior as we transition from weakly to strongly interacting systems. Observing these 1D behaviors requires extreme confinemnt.  Previous attempts have utilized templated porous glasses, created by organizing rod-like micelles into a triangular lattice within a silica matrix. These materials offer high aspect ratios and large sample volumes suitable for neutron scattering studies. However, they face a fundamental limitation - the minimum diameter of the pores is typically constrained by the micelle size ($1.5$–$2.0$ nm). This is significantly larger than the helium correlation length. Consequently, helium adsorbed directly into these matrices continues to exhibit bulk-like or 3D behavior rather than the desired 1D dynamics.\\

\noindent
We have recently developed a nanoengineering technique that enables us to observe Luttinger liquid behavior in $^4$He. By preplating the pores of a templated glass with argon at high temperatures, we can effectively reduce the pore diameter, allowing confined $^4$He to enter the Luttinger liquid regime. In this paper, we will review previous studies of confined $^4$He that led to the observation of Luttinger liquid behavior in liquid helium.\\

\section{Background}\label{sec2}

\noindent
Porous materials, such as vycor and aerogel, have been a popular medium for studying the effects of reduced dimensionality on helium.  MCM-41 is a mesoporous silicate molecular sieve, synthesized from rod-like micelles which form a close-packed triangular array in an aqueous silica solution.  The silica condenses to form a solid structure and the micelles are removed via calcination to create the templated glass. Its key characteristics include well-defined hexagonal pores, a narrow pore size distribution, minimal pore networking or pore blocking effects, and a high degree of pore ordering over micrometers length scale. Additionally, MCM-41 exhibits remarkable thermal, hydrothermal, chemical, and mechanical stability \cite{selvam2001recent}. The resulting material has pore diameters in the 2-4 nm range.\\

\noindent
When confined in pores much larger than the helium correlation length the helium consists of three distinct regions.  First, a solid forms at the pore wall.  On top of the solid layer a liquid layer forms with a density higher than that of the bulk liquid.  Finally, a bulk like liquid forms at the center of the pore. The high density liquid and the bulk like liquid have different excitations spectrums and excitations, such as rotons, are not able to pass between these layers due the energy-momentum mismatch.  This is the same mechanism that gives rise thermal Kapitza resistance for heat transfer between dissimalr materials.  Thus, these larger pore templated glasses have been likened to fiber optic cables, but for rotons.\\

\noindent
The physical limitations on the synthesis of tempalted porous materials limits the pore radii greater than $\approx$ 20 \AA, Thus, the liquid that that forms in the center of the  1D channels is always a bulk-like 3D liquid.  Nichol's et. al. proposed an active nanoengineering solution to this problem by preplating MCM-41 with a single, well controlled layer of Ar gas before filling the pores with helium. The Argon would be adsorbed to the pore walls at 80 K and would be solid-like at 4 K where studies could be carried out. Calculations of the adsorption potential for a single helium interacting with the Ar preplated MCM-41 indicated that preplating had two effects. First, it reduced the pore radius from $15 \AA$ to  $ 10 \AA$. Secondly, it significantly softened the adsorption potential at the pore wall, reducing this from $\approx 170~K$ for bare MCM-41 to $\approx 70~K$.\\

\noindent
Nichols et. al. carried out large scale quantum Monte Carlo simulations to examine the structure of $^4$He adsorbed in the Ar-plated pores of MCM-41 with a radius of 15 Å. They found that the adsorbed helium formed in four distinct layers.  The first two layers fill almost immediately and are fully solid. The final two layers fill together but the density of the third layer is always higher than that of the final layer. This isolates the core layer from the remainder of the system due the mismatch in excitation energies. \\

\noindent
Del Maestro et. al. were subsequently able to use elastic and inelastic neu


